A Performance Evaluation of Nomon: A Flexible Interface for Noisy Single-Switch Users

Some individuals with motor impairments communicate using a single switch -- such as a button click, air puff, or blink. Row-column scanning provides a method for choosing items arranged in a grid using a single switch. An alternative, Nomon, allows potential selections to be arranged arbitrarily rather than requiring a grid (as desired for gaming, drawing, etc.) -- and provides an alternative probabilistic selection method. While past results suggest that Nomon may be faster and easier to use than row-column scanning, no work has yet quantified performance of the two methods over longer time periods or in tasks beyond writing. In this paper, we also develop and validate a webcam-based switch that allows a user without a motor impairment to approximate the response times of a motor-impaired single switch user; although the approximation is not a replacement for testing with single-switch users, it allows us to better initialize, calibrate, and evaluate our method. Over 10 sessions with the webcam switch, we found users typed faster and more easily with Nomon than with row-column scanning. The benefits of Nomon were even more pronounced in a picture-selection task. Evaluation and feedback from a motor-impaired switch user further supports the promise of Nomon.

==> background.tex <==
%\susection{Background} \label{section:Background}

\subsection{Row Column Scanning Systems}
A common method of single-switch communication is row-column scanning (RCS). In RCS, the user is presented with a 2D array of options from which that they can select. For text composition, these options are letters and word completions. As depicted in Figure \ref{figure:Row Column Scanning Keyboard Interface}, options are arranged into rows and columns that can be selected incrementally. The RCS software scans through each row at a constant time interval: the scan delay. When a user sends a switch input, or click, into the software, it selects the currently highlighted row and proceeds to scan through each column. The user clic{redh} selects the option. 
\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\linewidth]{figures/rowcol_capture_paper.PNG}
	\caption{Our row column scanning keyboard interface. To type, the user finds their desired word or character in the 2D array of options. The interface scans through rows at a constant time interval. When a user clicks their switch, it selects the currently highlighted row and starts scanning through columns. The user clicks again when their desired target is highlighted. Pictured above is our study interface in which participants copied a phrase displayed in the text box. The participant is partway through typing the phrase. The top row shows likely words based on their current word input of ``a''.}
	\label{figure:Row Column Scanning Keyboard Interface}
\end{figure}
\subsection{Nomon}
Nomon is an alternative method for single-switch communication \cite{nomonthesis, nomonjournal}. In Nomon, every option in the interface has a clock positioned next to it (Figure \ref{fig_teaser}). Each clock has a unique phase, and the minute hands of all clocks rotate at a constant speed. A user can adjust the rotation speed based on their perceptual and motor abilities. A user need only look at one clock to select its corresponding target.  Other methods like RCS require a user to shift their visual attention between different parts of the screen. The user is instructed to click when the clock hand passes the red ``noon'' line. After each click, the clock hands change phase. The phase change is done to separate the clock phases of the most probable next targets from one another. The user repeatedly clicks when the minute hand passes noon until their target is selected. The number of clicks required to select an option is dependent on the precision of the user and on how probable the user's target is. In a keyboard application that makes use of a language model (as in Figure \ref{fig_teaser}), an experienced user can select targets in around two clicks\cite{nomonjournal}.


\subsection{Comparison}
\label{subsection:Comparison}
A key difference between RCS and Nomon is that RCS interfaces are typically deterministic while Nomon is probabilistic in operation. This probabilistic mechanism is what allows Nomon to adapt to users click ability and ensure they can select targets as efficiently as possible. RCS systems operate under a predetermined sequence of scans and always require two clicks per selection. These systems assume an ideal user who always clicks at the correct time. Therefore, a single imprecise click can result in an incorrect selection that can be time consuming to undo. Nomon, on the other hand, incorporates prior information and a model of user-input noise to adapt its selection criteria to a user's ability. In the keyboard application, each clock is assigned a prior according to Nomon's language model. Users rarely press exactly at noon on a given clock. Nomon models the observed click time as a random sample from a user's click distribution --- a likelihood over observed click times relative to noon. Nomon then computes the posterior distribution over all options from the prior and likelihood estimates, conditioned on the observed click times. A target is selected when the maximum posterior probability of any target exceeds the target with the second highest probability by a set threshold. As such, there is no fixed number of clicks required to make a selection in Nomon: the number of clicks is dependent on the precision of the user and on the prior distribution over targets\cite{nomonthesis}.
